Retrieval Models Aren't Tool-Savvy: Benchmarking Tool Retrieval for Large Language Models

Tool learning aims to augment large language models (LLMs) with diverse tools, enabling them to act as agents for solving practical tasks. Due to the limited context length of tool-using LLMs, adopting information retrieval (IR) models to select useful tools from large toolsets is a critical initial step. However, the performance of IR models in tool retrieval tasks remains underexplored and unclear. Most tool-use benchmarks simplify this step by manually pre-annotating a small set of relevant tools for each task, which is far from the real-world scenarios. In this paper, we propose ToolRet, a heterogeneous tool retrieval benchmark comprising 7.6k diverse retrieval tasks, and a corpus of 43k tools, collected from existing datasets. We benchmark six types of models on ToolRet. Surprisingly, even the models with strong performance in conventional IR benchmarks, exhibit poor performance on ToolRet. This low retrieval quality degrades the task pass rate of tool-use LLMs. As a further step, we contribute a large-scale training dataset with over 200k instances, which substantially optimizes the tool retrieval ability of IR models.

==> preamble/authors.tex <==
\author{First Author \\
  Affiliation / Address line 1 \\
  Affiliation / Address line 2 \\
  Affiliation / Address line 3 \\
  \texttt{email@domain} \\\And
  Second Author \\
  Affiliation / Address line 1 \\
  Affiliation / Address line 2 \\
  Affiliation / Address line 3 \\
  \texttt{email@domain} \\}

==> table/human.tex <==
\begin{table}[!t]
\centering
\begin{adjustbox}{width=2\columnwidth,center}
\begin{tabular}{@{} r@{} p{14cm} }
\toprule
\begin{tabular}[c]{@{}c@{}} \textbf{Quality Review Question} \end{tabular}    
% & \textbf{\changed{Mechanism}} 
&\begin{tabular}[c]{@{}c@{}} Yes or No \% \end{tabular}    
\\
\cmidrule(r){1-1}
\cmidrule(r){2-2}

% 
\code{ToolBench}~\cite{qin2023toolllm}
& 
\\


\specialrule{0em}{1pt}{1pt}
\cdashline{1-2}[6pt/6pt]
\specialrule{0em}{1pt}{1pt}

%
\textit{Whether the instruction describes the feature of target tools}
 & \multirow{2}{*}{ 92.3\% / 8.7\%}    
\\


\specialrule{0em}{1pt}{1pt}
\cdashline{1-2}[6pt/6pt]
\specialrule{0em}{1pt}{1pt}

\textit{Whether the instruction comprehensively describe the feature of all target tools} 
&  \multirow{2}{*}{ 89.2\% / 10.8\%}   
\\

\specialrule{0em}{1pt}{1pt}
\cdashline{1-2}[6pt/6pt]
\specialrule{0em}{1pt}{1pt}

\textit{Whether the instruction contains hallucination about the target tools or input query?}
& 
 \multirow{3}{*}{ 5.9\% / 94.1\%}  
\\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{The  quality review for our generated instructions, where the four questions are reviewed by three well-educated masters with 0.743 \textit{Kappa} statistics.}
\label{tab:dataset}
\end{table}

==> table/test.tex <==
\definecolor{backred}{RGB}{255, 190, 190}
\definecolor{backblue}{RGB}{220, 230, 250}
\newcommand{\red}[1]{\textcolor{red}{\textbf{#1}}}
\newtcbox{\hlprimarytab}{on line, rounded corners, box align=base, colback=backblue, colframe=white, size=fbox, arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}
\newtcbox{\hlsecondarytab}{on line, box align=base, colback=backred, colframe=white, size=fbox, arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}

\newcommand{\besttext}[1]{{\hlsecondarytab{#1}}}
\newcommand{\hightext}[1]{{\hlprimarytab{#1}}}

% \definecolor{backblue}{RGB}{208, 230, 251}
\newcommand{\best}{\cellcolor{backred}\textbf}
\newcommand{\high}{\cellcolor{backblue}\textbf}

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l| cc cc cc cc cc cc cc@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{I1-Inst.}}
 & \multicolumn{2}{c}{\textbf{I1-Tool}}
 & \multicolumn{2}{c}{\textbf{I1-Cat.}} 
 & \multicolumn{2}{c}{\textbf{I2-Inst.}} 
 & \multicolumn{2}{c}{\textbf{I2-Cat.}} 
 & \multicolumn{2}{c}{\textbf{I3-Inst.}} 
 & \multicolumn{2}{c}{\textbf{Average}}
 \\ \cmidrule(l){2-15} 
\multirow{-2}{*}{\textbf{Method}} 
& SoPR & \multicolumn{1}{c|}{SoWR}
& SoPR & \multicolumn{1}{c|}{SoWR}
& SoPR & \multicolumn{1}{c|}{SoWR}
& SoPR & \multicolumn{1}{c|}{SoWR} 
& SoPR & \multicolumn{1}{c|}{SoWR}
& SoPR & \multicolumn{1}{c|}{SoWR} 
& SoPR & SoWR \\
\hline
\rowcolor{Gainsboro} \multicolumn{15}{c}{\textit{GPT-series}} \\
\midrule 
\specialrule{0em}{1pt}{1pt}

GPT-3.5 (CoT)
& 53.0 & \multicolumn{1}{c|}{--} 
& 53.0 & \multicolumn{1}{c|}{--}
& 51.2 & \multicolumn{1}{c|}{--}
& 37.6 & \multicolumn{1}{c|}{--} 
& 43.9 & \multicolumn{1}{c|}{--}
& 48.6 & \multicolumn{1}{c|}{--} 
& 47.9 & - \\

GPT-3.5 (DFSDT) 
& 63.8 & \multicolumn{1}{c|}{58.9}
& 73.9 & \multicolumn{1}{c|}{65.8}
& 65.8 & \multicolumn{1}{c|}{60.1}
& 57.1 & \multicolumn{1}{c|}{72.6} 
& 69.8 & \multicolumn{1}{c|}{68.5} 
& 69.9 & \multicolumn{1}{c|}{67.2} 
& 66.7 & 65.5 \\

GPT-3.5 (Parallel) 
& 64.6 & \multicolumn{1}{c|}{48.5}
& 65.0 & \multicolumn{1}{c|}{55.7} 
& 69.0 & \multicolumn{1}{c|}{54.2}
& 54.9 & \multicolumn{1}{c|}{55.7}
& 61.4 & \multicolumn{1}{c|}{53.2}
& 56.6 & \multicolumn{1}{c|}{50.8} 
& 61.9 & 53.0 \\

GPT-4 (CoT) 
& 54.4 & \multicolumn{1}{c|}{53.4}
& 44.1 & \multicolumn{1}{c|}{60.1} 
& 48.8 & \multicolumn{1}{c|}{52.9} 
& 50.6 & \multicolumn{1}{c|}{69.8} 
& 48.9 & \multicolumn{1}{c|}{62.1}
& 42.6 & \multicolumn{1}{c|}{54.1}
& 48.2 & 58.7 \\

GPT-4 (DFSDT) 
& \best{69.0} & \multicolumn{1}{c|}{57.1} 
& \best{69.6} & \multicolumn{1}{c|}{\best{66.5}}
& 68.1 & \multicolumn{1}{c|}{61.4} 
& 70.8 & \multicolumn{1}{c|}{73.6} 
& 68.0 & \multicolumn{1}{c|}{62.9}
& \best{76.0 }& \multicolumn{1}{c|}{63.9} 
&  \best{70.3} & 64.2 \\

GPT-4 (Parallel) 
& 62.9 & \multicolumn{1}{c|}{\best{66.3}} 
& 67.4 & \multicolumn{1}{c|}{61.4} 
& \best{70.9} & \multicolumn{1}{c|}{\best{62.7}}
&  \best{73.4} & \multicolumn{1}{c|}{\best{85.8}}
& \best{70.8} & \multicolumn{1}{c|}{\best{77.4}}
& 69.7 & \multicolumn{1}{c|}{\best{70.5}} 
& 69.2 &  \best{70.7} \\
\hline

\rowcolor{Gainsboro} \multicolumn{15}{c}{\textit{Open-source}} \\
\midrule
\specialrule{0em}{1pt}{1pt}

ToolLLaMA (CoT)
& 42.7 & \multicolumn{1}{c|}{36.2}
& 35.4 & \multicolumn{1}{c|}{36.1}
& 38.6 & \multicolumn{1}{c|}{34.6} 
& 39.9 & \multicolumn{1}{c|}{49.1}
& 40.9 & \multicolumn{1}{c|}{38.7} 
& 29.8 & \multicolumn{1}{c|}{41.0}
& 37.9 & 39.3 \\

ToolLLaMA (DFSDT)
& 56.6 & \multicolumn{1}{c|}{39.9} 
& 55.5 & \multicolumn{1}{c|}{46.8} 
& 56.5 & \multicolumn{1}{c|}{41.8}
& 49.7 & \multicolumn{1}{c|}{53.8}
& 53.4 & \multicolumn{1}{c|}{49.2} 
& 53.6 & \multicolumn{1}{c|}{50.8}
& 54.2 & 47.1 \\

ToolLLaMA (CoT$\dag$)
& 26.7 & \multicolumn{1}{c|}{22.1} 
& 25.0 & \multicolumn{1}{c|}{27.2}
& 31.7 & \multicolumn{1}{c|}{29.4}
& 23.1 & \multicolumn{1}{c|}{32.1} 
& 24.5 & \multicolumn{1}{c|}{28.2}
& 20.5 & \multicolumn{1}{c|}{24.6} 
& 25.3 & 27.3 \\

ToolLLaMA (DFSDT$\dag$) 
& 41.8 & \multicolumn{1}{c|}{35.6} 
& 39.9 & \multicolumn{1}{c|}{37.3}
& 44.9 & \multicolumn{1}{c|}{39.9}
& 36.0 & \multicolumn{1}{c|}{47.2} 
& 39.1 & \multicolumn{1}{c|}{39.5} 
& 33.3 & \multicolumn{1}{c|}{26.2} 
& 39.2 & 37.6 \\

Ours 
&\high{63.5} & \multicolumn{1}{c|}{\high{52.1} }
& \high{64.2} & \multicolumn{1}{c|}{\high{53.2}}
& \high{67.2} & \multicolumn{1}{c|}{\high{54.2}}
& \high{62.1} & \multicolumn{1}{c|}{\high{70.8} }
&  \high{71.9} & \multicolumn{1}{c|}{\high{65.3}}
& \high{67.5}  & \multicolumn{1}{c|}{\high{59.0}}
& \high{66.1} & \high{59.1} \\
\bottomrule
\end{tabular}
}
\caption{A comparison different baselines and method on StableToolBench. Considering that real-world APIs are time-sensitive, the results of baselines presented in the table are reproduced during the period \texttt{from September to October 2024} using their official implementation. We highlight the best performance of open-source models and GPT-series models with the \besttext{red} and \hightext{blue}, respectively.}
\label{tab:main}
\end{table*}

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l ccccccc}
\toprule
\textbf{Method} & ReAct & DFSDT & ReAct$\dag$  & DFSDT$\dag$ & Ours \\
\toprule
\rowcolor{Gainsboro}  \multicolumn{6}{c}{Inference latency (s)} \\
\midrule
\textbf{I1-Inst.}  &  33.66  & 75.62$_{\downarrow 114\%}$   & 54.00$_{\downarrow 59\%}$   &  113.00$_{\downarrow 232\%}$   &  \high{29.22$_\mathbf{\uparrow 15\%}$}  \\
\textbf{I1-Tool}    &  34.92   & 89.54$_{\downarrow 158\%}$  & 94.00$_{\downarrow 43\%}$    &  146.00$_{\downarrow 220\%}$    & \high{28.22$_\mathbf{\uparrow 17\%}$} \\
\textbf{I1-Cat.}  &  39.65  &  102.99$_{\downarrow 157\%}$   &  57.00$_{\downarrow 169\%}$   & 128.00$_{\downarrow 317\%}$    & \high{32.65$_\mathbf{\uparrow 17\%}$} \\
\textbf{I2-Inst.}  &   38.44  & 123.87$_{\downarrow 182\%}$    & 52.00$_{\downarrow 44\%}$   & 140.00$_{\downarrow 162\%}$    & \high{30.43$_\mathbf{\uparrow 26\%}$} \\
\textbf{I2-Cat.}  &  38.57   &  110.21$_{\downarrow 226\%}$   &  56.00$_{\downarrow 37\%}$   & 102.00$_{\downarrow 268\%}$    &   \high{29.20$_\mathbf{\uparrow 21\%}$} \\
\textbf{I3-Inst.}  &  45.96  & 119.93$_{\downarrow 161\%}$    & 81.00$_{\downarrow 76\%}$   & 139.00$_{\downarrow 202\%}$    &  \high{40.07$_\mathbf{\uparrow 13\%}$} \\
\textbf{Avg.}  &    & $_{\downarrow 167\%}$ & $_{\downarrow 69\%}$ &  $_{\downarrow 228\%}$ &  \high{$_{\downarrow 18\%}$} \\
\bottomrule
\rowcolor{Gainsboro}  \multicolumn{6}{c}{{ Speed up (rate)}} \\
\midrule 
\textbf{I1-Inst.}  &  1.00  & $\times$0.45  &  $\times$0.63  &  $\times$0.30  &  \high{$\times$1.18} \\
\textbf{I1-Tool}   & 1.00    & $\times$0.39  &  $\times$0.70  &  $\times$0.31  &  \high{$\times$1.20} \\
\textbf{I1-Cat.} &   1.00  & $\times$0.39  &  $\times$0.37  &  $\times$0.24  &   \high{$\times$1.20} \\
\textbf{I2-Inst.} &   1.00  &  $\times$0.35  &  $\times$0.69  &  $\times$0.38  &  \high{$\times$1.35} \\
\textbf{I2-Cat.} &   1.00  & $\times$0.31  &  $\times$0.73  &  $\times$0.27  &  \high{ $\times$1.27 }\\
\textbf{I3-Inst.} &   1.00  & $\times$0.38  &  $\times$0.57  &  $\times$0.33  &  \high{$\times$1.15}  \\
\textbf{Avg.} &   1.00  & $\times$0.37  &  $\times$0.59  &  $\times$0.3  &  \high{$\times$1.22} \\
\bottomrule

\end{tabular}
}
\caption{The table presents a comparison of the inference times of LLMs. Using the average inference time of ToolLLaMA (CoT) as a benchmark, other LLMs are represented by corresponding multiples, labeled as x.}
\label{tab:time}
\end{table}



==> table/token.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lc|cccccccccccccc@{}}
\toprule
\multicolumn{2}{l|}{} & \multicolumn{2}{c}{\textbf{I1-Inst.}} & \multicolumn{2}{c}{\textbf{I1-Tool}} & \multicolumn{2}{c}{\textbf{I1-Cat.}} & \multicolumn{2}{c}{\textbf{I2-Inst.}} & \multicolumn{2}{c}{\textbf{I2-Cat.}} & \multicolumn{2}{c}{\textbf{I3-Inst.}} & \multicolumn{2}{c}{\textbf{Average}}
\\ \cmidrule(l){3-16} 
\multicolumn{2}{l|}{\multirow{-2}{*}{\textbf{Method}}} 
& C. & \multicolumn{1}{c|}{P.} & C. & \multicolumn{1}{c|}{P.} 
& C. & \multicolumn{1}{c|}{P.} & C. & \multicolumn{1}{c|}{P.} 
& C. & \multicolumn{1}{c|}{P.} & C. & \multicolumn{1}{c|}{P.}
& C. & P. \\
\hline
\rowcolor{Gainsboro}  \multicolumn{16}{c}{\textit{GPT-series}} \\
\midrule 
 & Avg. & {\color[HTML]{FE0000} 0.3} & \multicolumn{1}{c|}{5.7} & {\color[HTML]{FE0000} 0.3} & \multicolumn{1}{c|}{7.2} & {\color[HTML]{FE0000} 0.2} & \multicolumn{1}{c|}{5.6} & {\color[HTML]{FE0000} 0.2} & \multicolumn{1}{c|}{7.9} & {\color[HTML]{FE0000} 0.2} & \multicolumn{1}{c|}{7.7} & {\color[HTML]{FE0000} 0.3} & \multicolumn{1}{c|}{9.7} & {\color[HTML]{FE0000} 0.3} & 7.3 \\
\multirow{-2}{*}{GPT-3.5 (CoT)} & Max. & 1.3 & \multicolumn{1}{c|}{17.1} & 1.9 & \multicolumn{1}{c|}{42.8} & 2.1 & \multicolumn{1}{c|}{\color[HTML]{FE0000} 14.7} & 1.5 & \multicolumn{1}{c|}{16.1} & 1.5 & \multicolumn{1}{c|}{17.6} & \color[HTML]{FE0000} 0.9 & \multicolumn{1}{c|}{23.7} & 1.5 & 22.0 \\ \midrule
 & Avg. & 1.1 & \multicolumn{1}{c|}{20.9} & 1.3 & \multicolumn{1}{c|}{27.9} & 1.2 & \multicolumn{1}{c|}{22.5} & 1.6 & \multicolumn{1}{c|}{34.6} & 1.4 & \multicolumn{1}{c|}{28.3} & 1.2 & \multicolumn{1}{c|}{26.2} & 1.3 & 26.7 \\
\multirow{-2}{*}{GPT-3.5 (DFSDT)} & Max. & 7.7 & \multicolumn{1}{c|}{171.7} & 10.0 & \multicolumn{1}{c|}{496.0} & 12.8 & \multicolumn{1}{c|}{296.7} & 7.9 & \multicolumn{1}{c|}{158.8} & 13.3 & \multicolumn{1}{c|}{194.0} & 10.1 & \multicolumn{1}{c|}{280.1} & 10.3 & 266.2 \\ \midrule
 & Avg. & 2.9 & \multicolumn{1}{c|}{42.8} & 3.2 & \multicolumn{1}{c|}{53.6} & 2.8 & \multicolumn{1}{c|}{42.7} & 3.3 & \multicolumn{1}{c|}{58.1} & 3..6 & \multicolumn{1}{c|}{59.6} & 4.5 & \multicolumn{1}{c|}{77.5} & 3.3 & 55.7 \\
\multirow{-2}{*}{GPT-3.5 (Parallel)} & Max. & 20.1 & \multicolumn{1}{c|}{321.9} & 30.5 & \multicolumn{1}{c|}{578.6} & 15.7 & \multicolumn{1}{c|}{252.6} & 16.0 & \multicolumn{1}{c|}{261.2} & 19.5 & \multicolumn{1}{c|}{297.1} & 17.3 & \multicolumn{1}{c|}{322.8} & 19.9 & 325.3 \\ \midrule
 & Avg. & 0.4 & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 4.3}} & 0.4 & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 5.3}} & 0.4 & \multicolumn{1}{c|}{4.6} & 0.5 & \multicolumn{1}{c|}{6.1} & 0.5 & \multicolumn{1}{c|}{6.1} & 0.5 & \multicolumn{1}{c|}{7.5} & 0.5 & 5.7 \\
\multirow{-2}{*}{GPT-4 (CoT)} & Max. & \color[HTML]{FE0000} 1.2 & \multicolumn{1}{c|}{\color[HTML]{FE0000} 15.8} & \color[HTML]{FE0000} 1.2 & \multicolumn{1}{c|}{43.6} & \color[HTML]{FE0000} 0.9 & \multicolumn{1}{c|}{17.9} & 1.3 & \multicolumn{1}{c|}{23.9} & 1.5 & \multicolumn{1}{c|}{23.7} & 0.9 & \multicolumn{1}{c|}{33.7} & \color[HTML]{FE0000} 1.2 & 26.4 \\ \midrule
 & Avg. & 0.8 & \multicolumn{1}{c|}{9.0} & 1.0 & \multicolumn{1}{c|}{13.5} & 0.9 & \multicolumn{1}{c|}{9.5} & 1.1 & \multicolumn{1}{c|}{17.5} & 1.5 & \multicolumn{1}{c|}{30.8} & 1.6 & \multicolumn{1}{c|}{30.4} & 1.2 & 18.5 \\
\multirow{-2}{*}{GPT-4 (DFSDT)} & Max. & 6.0 & \multicolumn{1}{c|}{109.4} & 10.1 & \multicolumn{1}{c|}{301.2} & 4.9 & \multicolumn{1}{c|}{114.2} & 11.3 & \multicolumn{1}{c|}{354.1} & 16.2 & \multicolumn{1}{c|}{380.2} & 13.2 & \multicolumn{1}{c|}{649.5} & 10.3 & 318.1 \\ \midrule
 & Avg. & 0.7 & \multicolumn{1}{c|}{6.0} & 1.2 & \multicolumn{1}{c|}{17.1} & 1.2 & \multicolumn{1}{c|}{18.7} & 0.7 & \multicolumn{1}{c|}{5.6} & 0.9 & \multicolumn{1}{c|}{9.7} & 1.4 & \multicolumn{1}{c|}{18.4} & 1.0 & 12.6 \\
\multirow{-2}{*}{GPT-4 (Parallel)} & Max. & 5.0 & \multicolumn{1}{c|}{88.5} & 19.4 & \multicolumn{1}{c|}{482.2} & 21.6 & \multicolumn{1}{c|}{440.8} & 4.0 & \multicolumn{1}{c|}{46.2} & 4.6 & \multicolumn{1}{c|}{118.8} & 13.9 & \multicolumn{1}{c|}{231.0} & 11.4 & 234.6 \\
\hline
\rowcolor{Gainsboro}\multicolumn{16}{c}{\textit{Open-source}} \\
\midrule
 & Avg. & 0.6 & \multicolumn{1}{c|}{6.4} & 0.5 & \multicolumn{1}{c|}{7.1} & 0.5 & \multicolumn{1}{c|}{5.8} & 0.6 & \multicolumn{1}{c|}{7.8} & 0.6 & \multicolumn{1}{c|}{7.4} & 0.6 & \multicolumn{1}{c|}{8.5} & 0.6 & 7.2 \\
\multirow{-2}{*}{ToolLLaMA (CoT)} & Max. & \underline{1.5} & \multicolumn{1}{c|}{21.2} & \underline{1.5} & \multicolumn{1}{c|}{41.3} & \underline{1.6} & \multicolumn{1}{c|}{\underline{17.7}} & 1.3 & \multicolumn{1}{c|}{14.8} & 1.4 & \multicolumn{1}{c|}{18.4} & 1.5 & \multicolumn{1}{c|}{18.7} & 1.5 & 22.0 \\ \midrule
 & Avg. & 1.3 & \multicolumn{1}{c|}{19.6} & 1.4 & \multicolumn{1}{c|}{22.7} & 1.2 & \multicolumn{1}{c|}{18.2} & 1.5 & \multicolumn{1}{c|}{27.8} & 1.5 & \multicolumn{1}{c|}{26.9} & 1.4 & \multicolumn{1}{c|}{23.8} & 1.4 & 23.2 \\
\multirow{-2}{*}{ToolLLaMA (DFSDT)} & Max. & 5.0 & \multicolumn{1}{c|}{96.4} & 8.4 & \multicolumn{1}{c|}{138.5} & 7.8 & \multicolumn{1}{c|}{118.0} & 4.6 & \multicolumn{1}{c|}{113.7} & 6.6 & \multicolumn{1}{c|}{106.5} & 4.4 & \multicolumn{1}{c|}{99.8} & 6.1 & 112.2 \\ \midrule
 & Avg. & 0.5 & \multicolumn{1}{c|}{6.7} & 0.5 & \multicolumn{1}{c|}{7.2} & \underline{0.4} & \multicolumn{1}{c|}{5.9} & 0.5 & \multicolumn{1}{c|}{7.8} & \underline{0.4} & \multicolumn{1}{c|}{7.6} & \underline{0.4} & \multicolumn{1}{c|}{8.2} & 0.5 & 7.2 \\
\multirow{-2}{*}{ToolLLaMA (CoT$\dag$)} & Max. & 2.0 & \multicolumn{1}{c|}{\underline{20.3}} & 1.8 & \multicolumn{1}{c|}{\underline{\color[HTML]{FE0000} 30.5}} & 1.7 & \multicolumn{1}{c|}{18.3} & \underline{\color[HTML]{FE0000} 1.3} & \multicolumn{1}{c|}{\underline{\color[HTML]{FE0000} 13.0}} & \underline{\color[HTML]{FE0000} 1.1} & \multicolumn{1}{c|}{\underline{\color[HTML]{FE0000} 17.2}} & \underline{1.2} & \multicolumn{1}{c|}{\underline{\color[HTML]{FE0000} 18.4}} & \underline{1.5} & \underline{\color[HTML]{FE0000} 19.6} \\ \midrule
 & Avg. & 1.3 & \multicolumn{1}{c|}{25.1} & 1.3 & \multicolumn{1}{c|}{24.3} & 1.1 & \multicolumn{1}{c|}{19.7} & 1.2 & \multicolumn{1}{c|}{24.1} & 1.3 & \multicolumn{1}{c|}{29.6} & 1.0 & \multicolumn{1}{c|}{19.4} & 1.2 & 23.7 \\
\multirow{-2}{*}{ToolLLaMA (DFSDT$\dag$)} & Max. & 15.3 & \multicolumn{1}{c|}{201.4} & 13.5 & \multicolumn{1}{c|}{175.6} & 12.1 & \multicolumn{1}{c|}{150.8} & 3.9 & \multicolumn{1}{c|}{105.9} & 4.5 & \multicolumn{1}{c|}{125.0} & 3.6 & \multicolumn{1}{c|}{70.8} & 8.8 & 138.3 \\ \midrule
 & Avg. & \underline{0.5} & \multicolumn{1}{c|}{\underline{4.8}} & \underline{0.5} & \multicolumn{1}{c|}{\underline{5.4}} & 0.5 & \multicolumn{1}{c|}{\underline{{\color[HTML]{FE0000} 4.6}}} & \underline{0.5} & \multicolumn{1}{c|}{{\underline{\color[HTML]{FE0000} 5.1}}} & 0.5 & \multicolumn{1}{c|}{{\underline{\color[HTML]{FE0000} 5.0}}} & 0.5 & \multicolumn{1}{c|}{\underline{\color[HTML]{FE0000} 6.3}} & \underline{0.5} & \underline{{\color[HTML]{FE0000} 5.2}} \\
\multirow{-2}{*}{Ours} & Max. & 1.8 & \multicolumn{1}{c|}{23.4} & 4.2 & \multicolumn{1}{c|}{59.8} & 4.4 & \multicolumn{1}{c|}{60.9} & 1.5 & \multicolumn{1}{c|}{29.5} & 1.4 & \multicolumn{1}{c|}{22.2} & 1.3 & \multicolumn{1}{c|}{25.3} & 2.4 & 36.9 \\ \bottomrule
\end{tabular}
}
\caption{The table shows the performance of various LLMs in terms of token consumption. All values in the table are expressed in thousands. On the horizontal axis, C. stands for \textit{Completion} and P. for \textit{Prompt}. On the vertical axis, Avg. indicates average and Max. represents the maximum. Similarly, {\color[HTML]{FE0000} red} indicates the best result in the entire column, while \underline{underline} denotes the best result in the open-source.}
\label{tab:token}
\end{table*}
